Periodic optimal control of nonlinear constrained systems using economic model predictive control

In this paper, we consider the problem of periodic optimal control of nonlinear systems subject to online changing and periodically time-varying economic performance measures using model predictive control (MPC). The proposed economic MPC scheme uses an online optimized artificial periodic orbit to ensure recursive feasibility and constraint satisfaction despite unpredictable changes in the economic performance index. We demonstrate that the direct extension of existing methods to periodic orbits does not necessarily yield the desirable closed-loop economic performance. Instead, we carefully revise the constraints on the artificial trajectory, which ensures that the closed-loop average performance is no worse than a locally optimal periodic orbit. In the special case that the prediction horizon is set to zero, the proposed scheme is a modified version of recent publications using periodicity constraints, with the important difference that the resulting closed loop has more degrees of freedom which are vital to ensure convergence to an optimal periodic orbit. In addition, we detail a tailored offline computation of suitable terminal ingredients, which are both theoretically and practically beneficial for closed-loop performance improvement. Finally, we demonstrate the practicality and performance improvements of the proposed approach on benchmark examples.

==> App_HVAC.tex <==
%!TEX root = ./EcoPeriodic.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Building cooling}
\label{app:HVAC} 


details 

$q_{amb}$, 
 
 constants...

==> Extensions_convex_periodic.tex <==
%!TEX root = ./EcoPeriodic.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsubsection{Strongly periodic problems}
\label{sec:convex_periodic}
In the following, we consider a special class of periodic optimal control problems, which are characterized by a strong dependence on the time-varying nature of $\ell,~f,~\mathcal{Z}_T$. 
%This special case, is not restricted to convex problems. 
%(Could also appear for nonlinear non-convex problems, if problem is dominated by time-varying nature) 
This strong dependence is characterized by the following assumption, which can be viewed as a stronger version of Assumption~\ref{ass:cont_orbit}. 
\begin{assumption}
\label{ass:cont_orbit_2}
There exists a positive constant $c_{\kappa}$, such that at any time step $t\in\mathbb{N}$, for any constant parameters $y(t)\in\mathbb{Y}$, and any state $x(t)$ with \eqref{eq:MPC} feasible, the following property holds: 
The solution to \eqref{eq:MPC} is equivalent to the solution of a simplified problem, where the constraints~\eqref{eq:kappa_con_1}--\eqref{eq:kappa_con_2} are replaced by $J_T(r(\cdot|t),t+N,y(t))\leq \kappa(t)$.  
\end{assumption}	
The following properties follow directly:\\
a) if Assumption~\ref{ass:cont_orbit_2} is satisfied, then we can use a simplified formulation that only needs a scalar memory state $\kappa(t)$, similar to the steady-state case in~\cite{muller2013economic,muller2014performance,fagiano2013generalized}. 
Furthermore, the number of (possibly nonlinear) inequality constraints in~\eqref{eq:MPC} is significantly reduced. \\
b) In a time-invariant setup ($\ell,~f,~V_f,~\mathcal{Z}_T$ independent of $t$), this assumption is in general not satisfied. 
In particular, whenever the optimal solution could be a shifted reference trajectory, compare example in Sec.~\ref{sec:pitfal}.\\
In case the problem is both time-invariant and convex, then the optimal operation is a steady-state. 

A thorough theoretical derivation of sufficient conditions for Assumption~\ref{ass:cont_orbit_2} is beyond the scope of this paper. 
However, we conjecture that this condition holds for linear systems with polytopic constraints and linear cost, which is also the case in of the numerical example in Section~\ref{sec:num}. 

 

==> Extensions_not_cont.tex <==
%!TEX root = ./EcoPeriodic.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Continuity condition not satisfied}
\label{sec:not_cont}
\textcolor{red}{Also have similar suboptimality analysis for Ass.~\ref{ass:cont_orbit} not satisfied. Not sure if relevant. Maybe short Remark.}
In the following, we briefly show, that in case the continuity condition (Ass.~\ref{ass:cont_orbit}) is not satisfied, the cost of the artificial periodic orbit converges to a value $\kappa_{\infty}$ which is arbitrary close to a local minimum of~\eqref{eq:opt_periodic}, for $c_{\kappa}$ sufficiently large.
Given boundedness of the stage cost $\ell$, define 
\begin{align*}
\ell_{\max}:=\sup_{t\in\mathbb{N},(x,u)\in\mathcal{Z}_r(t),(z,v)\in\mathcal{Z}_r(t),y\in\mathbb{Y}}\ell(x,u,t,y)-\ell(z,v,t,y).
\end{align*}
%
%Lemma~\ref{lemma:local_min}
The following proposition is an extension of Lemma~\ref{lemma:local_min} and Proposition~\ref{prop:art} to the case where Assumption~\ref{ass:cont_orbit} is \textit{not} satisfied. 
\begin{lemma}
\label{prop:art_2}
Let Assumptions \ref{ass:term_simple}, \ref{ass:term}, hold and assume that $y(t)\in\mathbb{Y}$ is constant. 
Assume that there exists a function $\alpha_{\eta}\in\mathcal{K}_{\infty}$, such that for any $t\in\mathbb{N}$, and any reference $r$ which is not a local minimizer to~\eqref{eq:opt_periodic}, there exists a local minimizer $\hat{r}$ to \eqref{eq:opt_periodic}, and a continuously parameterized family of reference trajectories $\tilde{r}^{\eta}$, $\eta\in[0,1]$, which satisfy $\|\tilde{r}^{\eta}-r\|\leq \alpha_{\eta}(\eta)$, 
\begin{align*}
J_T(\tilde{r}^{\eta},t,y)=(1-\eta)J_T(r,t,y)+\eta J_T(\hat{r},t,y). 
\end{align*}
Suppose that the optimization problem~\eqref{eq:MPC} is feasible at time $t$ with some reference trajectory $r^*(\cdot|t)$, which is not a local minimizer to~\eqref{eq:opt_periodic}. 
If the relative cost difference $\Delta J_T$ to the local minimizer $\hat{r}$ satisfies $\Delta J\geq \ell_{\max}\eta/c_{\kappa}$ with $\eta=\min\{1,\alpha_{\eta}^{-1}(\epsilon)\}$,
\begin{align*}
\Delta J_T=J_T(\mathcal{R}_Tr^*(\cdot|t),t,y)-J_T(\hat{r},t+1,y),
\end{align*}
 then the reference $\tilde{r}^{\eta}$ is a feasible solution to~\eqref{eq:MPC} at $t+1$. 
Furthermore, if the update rule $\mathcal{B}$ satisfies Assumption~\ref{ass:B1_2}, then there is a local minimum of~\eqref{eq:opt_periodic}, $J_{T,loc}$, such that $\kappa_{\infty}\leq J_{T,loc}+\ell_{\max}\eta/c_{\kappa}$. 
\end{lemma}
\begin{proof}
Abbreviate $J_{T}(r)=J_T(,t+N+1,y)$, $\Delta J_T=J_T(\tilde{r}_{\eta=0})-J_T(\tilde{r}_{\eta=1})$. 
Note, that the definition of $\ell_{\max}$ and $\Delta \kappa=J_{T}(\tilde{r}_{\eta=0})-J_{T}(\tilde{r}_{\eta})=\eta \Delta J_T$ ensures that this reference satisfies the constraints~\eqref{eq:kappa_con_1}--\eqref{eq:kappa_con_2}, with $c_{\kappa}\geq \ell_{\max}\eta \Delta J_T$. 
Furthermore, $\eta=\max\{\alpha_{\eta}^{-1}(\epsilon),1\}$ ensures $\|r-\tilde{r}\|\leq \epsilon$. 
Thus, similar to Lemma~\ref{lemma:local_min}, Lemma~\ref{lemma:change_r} the reference $\tilde{r}_{\eta}$ satisfies the constraints in~\eqref{eq:MPC}. 
Finally, convergence of $\kappa_{\infty}$ close to a local minimum of~\eqref{eq:opt_periodic} follows with the arguments in Proposition~\ref{prop:art}. 
\end{proof}
Given a continuity condition on the set of periodic trajectories $r$, this result ensures even if Assumption~\ref{ass:cont_orbit} is not satisfied, we can incrementally improve the cost of the artificial reference $J_T$ to a local minimum, up to tolerance $\ell_{\max}\eta/c_{\kappa}$, which can be made arbitrarily small by increasing $c_{\kappa}$.  
Note, that the performance bounds relative to $\kappa_{\infty}$ (Prop.~\ref{prop:av_perf}) are independent of Assumption~\ref{ass:cont_orbit}. 
Thus, even if this Assumption is not satisfied, for $c_{\kappa}$ sufficiently, this leads to an arbitrary small deterioration of the average performance. 


\begin{comment}

\subsubsection*{
\textbf{\textcolor{red}{Ass.~\ref{ass:cont_orbit} not even satisfied in linear unconstrained strongly convex case by gradient descent}}}
 gradient~\cite{boyd2004convex}. $r^+=r-\nabla J(r)/M$.\
\begin{align*}
c_{\kappa}(J_T(r^+)-J_T(r))\leq -c_{\kappa}/(2M)\|\nabla J_T(r)\|^2\\
\stackrel{!}{\leq} -L/m\|\nabla J_T(r)\|\\
\leq \ell(r^+)-\ell(r)
%\leq L_g\|x-x^+\|\leq L_g\|\nabla f(x)\|/M\\
% g(x)-g(x^+)\leq L_g\|x-x^+\|\leq L_g\|\nabla f(x)\|/M\\
\end{align*}
where $L$ is a local Lipschitz constant of $\ell$ and $M,m$ correspond to the strong convexity. \\
Condition satisfied for $c_{\kappa}\geq m/(2M L_g)/\|\nabla f(x)\|$.., cannot hold close to optimum...\\
Exception: if $\nabla J_T$ is not zero at the optiimum, i.e., then could possibly work with a different proof.\\
Also obviously satisfied if $\|\nabla \ell\|\sim\|\nabla J_T\|$, which i don't know how to verify. \\
\subsubsection*{\textbf{\textcolor{red}{Alternative formulation different $c_{\kappa}$}}}:
\begin{align*}
(\ell(r^+)-\ell(r))^2\leq c_{\kappa}\Delta J_T\\
\ell(r^+)\leq \ell(r)-c_{\kappa}\sqrt{\Delta \kappa}.
\end{align*} 
Problem a: for linear system with linear cost, this is a QCQP, but for $\ell$ quadratic it is non-standard...\\
Derivation~\eqref{eq:kappa_bound_1}
\begin{align*}
\kappa_j(t+1)\leq \kappa_{j+1}(t)-c_{\kappa}\sqrt{\Delta \kappa}\\
\kappa_{T-1}(t+k+1)\leq \kappa_{k}+c_{\kappa}\sum_{j=0}^{k}\sqrt{-\Delta\kappa(t+j)}\\
\sum_{k=0}^{T-1}\kappa_{T-1}(t+k+1)-\kappa_k(t)\leq c_{\kappa}T\sum_{k=0}^{T-1}\sqrt{-\Delta\kappa(t+k)}
\end{align*}
Note, that 
\begin{align*}
&\sqrt{a}+\sqrt{b}\leq \sqrt{2}\sqrt{a+b}\\
&\sqrt{a}+\sqrt{b}+\sqrt{c}+\sqrt{d}\\
\leq& \sqrt{2}(\sqrt{a+b}+\sqrt{c+d})\leq 2\sqrt{a+b+c+d}\\
&\sum_{k=1}^{2^3}\sqrt{a_k}\leq \sqrt{2}^3\sqrt{\sum_k a_k}\\
%\sqrt{a}+\sqrt{b}\geq \sqrt{a+b}.
&\sum_{k=0}^{T-1}\sqrt{-\Delta\kappa(t+k)}\leq \sqrt{T}\sqrt{\kappa(0)-\kappa(T)}.
\end{align*}
Thus, we have
\begin{align*}
\sum_{k=0}^{T-1}\kappa_{T-1}(t+k+1)-\kappa_k(t)\leq c_{\kappa}T\sqrt{T}\sqrt{\kappa(0)-\kappa(T)}.
\end{align*}
Finally, this yields
\begin{align*}
W(KT)-W(0)\leq K\kappa_{\infty}+c_{\kappa}T\sqrt{TK}\sqrt{\kappa(0)-\kappa(TK))}
\end{align*}
This bound becomes infinite...for $K$ large.
\end{comment}

\begin{comment}
\begin{lemma}
Let Assumptions \ref{ass:term_simple}, \ref{ass:term}, hold and assume that $y(t)$ is constant. 
Suppose that the optimization problem~\eqref{eq:MPC} is feasible at time $t$ with some reference trajectory $r^*(\cdot|t)$, which is not a local minimizer to~\eqref{eq:opt_periodic}. 

Assume that for  

Consider a local minimizer $\tilde{r}$ to~\eqref{eq:opt_periodic} with cost $\tilde{J_T}$. 
Consider a set of continously parameterized references $\tilde{r}^{\eta}\in\mathcal{Z}_T(t+N+1)$, $\eta\in[0,1]$ that connect $\mathcal{R}_Tr^*(\cdot|t)$ to $\tilde{r}$ with a linear change in the cost $J_T$, i.e.,  $J_T(\tilde{r}^{\eta},t+N+1,y)=(1-\eta)J_T(\tilde{r},t+N+1,y)+\eta J_T(\tilde{r},t+N+1,y)$. 
Assume that this set of trajectories is continous in $\eta$, i.e., there exists a function $\alpha_{\eta}\in\mathcal{K}_{\infty}$, such that $\|\tilde{r}_{\eta=0}-\tilde{r}_{\eta}\|\leq \alpha_{\eta}(\eta)$. %(J_T(r)-J_T(\tilde{r}_{\eta}))$.
Then for $c_{\kappa}\geq \ell_{\max}\eta/\Delta J_T$, the reference $\tilde{r}_{\eta}$ with $\eta=xx$  is a feasible candidate solution to~\eqref{eq:MPC} at $t+1$ and satisfies
\begin{align*}
j_T(\tilde{r})\leq J_T({r})-\eta(J_T-J_T)
\end{align*}
\end{lemma}
\end{comment}



\begin{comment}

%For simplicity, we consider the case, where the perodic optimal control problem~\eqref{eq:opt_periodic} has a unique minimum. 
%In addition, we reqire a continuity condition on the set of perodic orbits. 
\begin{assumption}
\label{ass:cont_eps}
%The perodic optimal control problem~\eqref{eq:opt_periodic} has a unique minimum.
There exists a function $\alpha_{\epsilon}\in\mathcal{K}_{\infty}s$, such that for any reference $r\in\mathcal{Z}_T(t)$, which is not a local minimizer of
~\eqref{eq:opt_periodic}.
There exists a continously parameterized set of references $\tilde{r}_{\eta}\in\mathcal{Z}_T(t)$, $\eta\in[0,1]$ with $\tilde{r}_{0}=r$ and $\tilde{r}_{1}$ a local mimimum.
The set of trajectories satisfy
% that improve cost $J_T$, with a bounded distance, i.e.,
 $\|r-\tilde{r}_{\eta}\|\leq \alpha_{\epsilon}(J_T(r)-J_T(\tilde{r}_{\eta}))$.
\end{assumption}




%not fruitful....s

\textbf{sufficient conditions continuity}
\begin{enumerate}
\item 1. suppose that stage cost is locally Lipschitz continous:
\begin{align*}
\ell(r+\Delta r)-\ell(r)\leq L_{\ell}\|\Delta r\|
\end{align*}
condition in Assumption~\ref{ass:cont_orbit} can be satisfied with
\begin{align*}
c_{\kappa}(J_T(r)-J_T(r+\Delta r))\geq L_{\ell}\|\Delta r\|\geq \ell(r)-\ell(r+\Delta r)
\end{align*}
\end{enumerate}

write as directed gradient
\begin{align*}
\nabla_{\Delta r} J=\sum_j\nabla_{\Delta r}\ell(j)\leq \nabla_{\Delta r}\ell(j)/c_{\kappa}
\end{align*}

convex, decrease\\
$f(r+\Delta r)\leq f(r)-m\|\Delta r\|^2$\\
\end{comment}


==> Literature.tex <==
%!TEX root = ./EcoPeriodic.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
\begin{itemize}
\item \cite{angeli2012average}: economic MPC, average cost
\item \cite{houska2017cost}: cost to travel, periodic 
\item \cite{wang2018economic}:similar linear, periodicity constraint, converges to periodic trajectory, optimal based on KKT\\
details: $\ell_k(x,u,p(k|t))$, most general, time-varying cost and time-varying and possibly changing price signal\\
here:periodiciy due to periodic price \quad alternative: periodicity even in time-invaraint setting~CSTR\\
remark 5: other periodic trajectories might also result, but special case $\rightarrow$ Rebutal: standard case, e.g. $T=1$\\
half of the paper is an application..., \quad there the MPC converges to optimal,\quad possible reason: over-actuated\\
not sure if also optimal in the second example

\item \cite{limon2014single}: artifical reference + tracking, linear systems
\item \cite{ferramosca2014economic}: artifical setpoint, linear
\item \cite{ferramosca2010economic}: artifical setpoint, nonlinear (not sure if correct...)
\item \cite{fagiano2013generalized}: artifical setpoint, nonlinear, not sure how terminal cost, controllabel
\item \cite{muller2013economic,muller2014performance}: artifical setpoint, nonlinear, terminal cost, self-tuning, performance-guarantees
\item \cite{muller2016economic}: economic MPC periodic without terminal
\item Given optimal periodic trajectory: use economic MPC:\\
\cite{zanon2017periodic}: periodic EMPC, dissipativiy
\item \cite{broomhead2015robust}: linear, nilpotent controllable, robust, periodic, ..., not necessarily interesting..., also uses periodic artifical reference + offset cost (predicted =economic, artifical =tracking/offset) $\rightarrow$ maybe special case
\item Time-varying economic cost~\cite{angeli2016theoretical}: optimal steady-state not computed by MPC, only changing deal with finite set of points, connecting trajectories computed offline\\
\item Terminal cost in EMPC\\
compute terminal cost:\cite{amrit2011economic}, extension of~\cite{chen1998quasi}\\
\cite{alessandretti2014economic}: continous-time, more general\\
\cite{alessandretti2016convergence}: given time-varying optimal trajectory: use terminal cost to get bounds (maybe extension of~\cite{zanon2017periodic})\\
contains formula for terminal cost based on exp. stability and exp. convergence,\quad explain how to do basd on linearization around one steady-state\\
\cite{alessandretti2016design}: discrete-time\\
%\cite{donganalysis}: analysis of more general dissip EMPC
%\item Examples: \\
%linear robust periodic economic - water: \cite{wang2017robust}
\end{itemize}
 
